A Study on Domain Generalization for Failure Detection through Human Reactions in HRI

Machine learning models are commonly tested in-distribution (same dataset); performance almost always drops in out-of-distribution settings. For HRI research, the goal is often to develop generalized models. This makes domain generalization - retaining performance in different settings - a critical issue. In this study, we present a concise analysis of domain generalization in failure detection models trained on human facial expressions. Using two distinct datasets of humans reacting to videos where error occurs, one from a controlled lab setting and another collected online, we trained deep learning models on each dataset. When testing these models on the alternate dataset, we observed a significant performance drop. We reflect on the causes for the observed model behavior and leave recommendations. This work emphasizes the need for HRI research focusing on improving model robustness and real-life applicability.

==> sections/_reviews_hriworkshop.tex <==
----------------------- REVIEW 1 ---------------------
SUBMISSION: 5
TITLE: A Study on Domain Generalization for Failure Detection through Human Reactions in HRI
AUTHORS: Maria Teresa Parreira, Sukruth Gowdru Lingaraju, Adolfo Ramirez-Aristizabal, Manaswi Saha, Michael Kuniavsky and Wendy Ju

----------- Overall evaluation -----------
SCORE: 3 (strong accept)
This workshop paper provides a preliminary evaluation of two distinct datasets---one obtained in a lab and the other online---examining human responses to robot errors and the consequent performance decline when these models are tested on alternate datasets for domain generalization. The paper is well-written and the discussion of the findings is insightful.
However, I would appreciate further discussion on:
1. Real-Time Detection: How can these findings be operationalized for real-time error detection? Considering the temporal dynamics of human reactions to errors is crucial. In case these errors are prolonged, how does this impact detection? Presenting results in terms of the number of errors identified, in addition to frame level, can offer a clearer understanding of the model's effectiveness in practical real-world scenarios. For example, if an error is detected in a few frames, lets say 3-4, because the error's intensity is sufficient for detection, or due to an optimal camera angle, this indicates correct error identification within that instance (clip). This could be true even if not all frames capture the error, which might have lower accuracy according to the current evaluation but can be operationalized in real-world. Such nuances are currently absent from discussion.

2. Consistency of Human Reactions: Particularly in prolonged error scenarios, human reactions may vary over time. Additionally, when the human subject is mobile, tracking facial expressions may not be feasible 100\% of the time during the erroneous interaction. It would be beneficial to see the authors' perspectives on how these factors might affect the operationalization of their evaluation.

3. First-Person Perspective in Human-Robot Collaboration: An analysis of how these findings translate to a first-person perspective from bystanders in human-robot collaboration would be intriguing. Understanding how the dynamics change from this viewpoint could provide valuable insights for practical applications.
